FedDefender: Client-Side Attack-Tolerant Federated Learning

Federated learning enables learning from decentralized data sources without compromising privacy, which makes it a crucial technique. However, it is vulnerable to model poisoning attacks, where malicious clients interfere with the training process. Previous defense mechanisms have focused on the server-side by using careful model aggregation, but this may not be effective when the data is not identically distributed or when attackers can access the information of benign clients. In this paper, we propose a new defense mechanism that focuses on the client-side, called FedDefender, to help benign clients train robust local models and avoid the adverse impact of malicious model updates from attackers, even when a server-side defense cannot identify or remove adversaries. Our method consists of two main components: (1) attack-tolerant local meta update and (2) attack-tolerant global knowledge distillation. These components are used to find noise-resilient model parameters while accurately extracting knowledge from a potentially corrupted global model. Our client-side defense strategy has a flexible structure and can work in conjunction with any existing server-side strategies. Evaluations of real-world scenarios across multiple datasets show that the proposed method enhances the robustness of federated learning against model poisoning attacks.

==> tables/attack_no_info_std.tex <==
\begin{table*}[b!]
{
\caption{Performance results on classification accuracy with standard errors in Scenario-1 over four datasets. Our model brings non-trivial improvement for all server-sied baseline algorithms for both last and best accuracy.}
\cutcationup
\label{tab:main_result_std}
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{CIFAR-10} &  \multicolumn{2}{c|}{CIFAR-100} & \multicolumn{2}{c|}{TinyImageNet} & \multicolumn{2}{c}{FEMNIST} \\ 
                      & ~~ Last ~~  & ~~ Best ~~  &  ~~ Last ~~ & ~~ Best ~~  & ~~ Last ~~ & ~~ Best ~~ & ~~ Last ~~ & ~~ Best ~~  \\ \midrule
No Defense            &   68.80 $\pm$ 3.58    &  71.96 $\pm$ 1.11  &  42.97 $\pm$ 1.29 & 43.90 $\pm$ 0.72  & 30.37 $\pm$ 3.56 & 38.98 $\pm$ 0.34 & 18.88 $\pm$ 1.51 & 23.81  $\pm$ 0.37 \\
+ \model{}           & \textbf{78.17 $\pm$ 2.20} & \textbf{79.96 $\pm$ 0.80 } & \textbf{51.76 $\pm$ 0.54}  & \textbf{51.92 $\pm$  0.33} &  \textbf{35.59 $\pm$ 2.52}  &  \textbf{39.68 $\pm$  0.24}  & \textbf{22.11 $\pm$  2.19} & \textbf{24.48 $\pm$ 0.28} \\ \hline
Median               &	62.02 $\pm$ 3.96 & 64.76 $\pm$ 1.41 & 36.33 $\pm$	0.97 & 37.54 $\pm$ 0.52 & 26.73 $\pm$ 3.79 & 32.53 $\pm$ 0.43 &12.00 $\pm$ 1.69 & 20.03 $\pm$ 0.64\\
+ \model{}            	&  \textbf{72.96 $\pm$ 3.99} & \textbf{76.28 $\pm$ 0.40} &  \textbf{39.89 $\pm$ 1.18} & \textbf{41.29 $\pm$ 0.91}  & \textbf{26.92 $\pm$ 3.74} & \textbf{32.88 $\pm$ 0.92} & \textbf{15.75 $\pm$ 2.84}  & \textbf{21.24 $\pm$ 0.86}  \\ \hline
Trimmed Mean                &  75.52 $\pm$ 1.78     & 76.03 $\pm$ 0.95   &  47.93 $\pm$ 0.40 & 47.95 $\pm$ 0.41 &  36.76 $\pm$ 0.59 & 38.24 $\pm$ 0.13 & 19.37 $\pm$ 2.27 & 23.17 $\pm$ 0.87 \\
+ \model{}           	  &    \textbf{81.06 $\pm$ 1.55}    &   \textbf{81.96 $\pm$ 0.60}   &  \textbf{52.90 $\pm$ 0.75}  & \textbf{53.41 $\pm$ 0.32}  & \textbf{38.85 $\pm$ 0.17}  &   \textbf{39.37 $\pm$ 0.14} & \textbf{21.80 $\pm$ 1.96} & \textbf{23.95 $\pm$ 0.07}\\ \hline
Norm Bound          	  &  67.36 $\pm$ 2.69       &  70.07 $\pm$ 0.99     &  42.51 $\pm$ 1.85   & 45.12 $\pm$ 0.51   &  30.78 $\pm$ 4.05  & 35.87 $\pm$ 0.17 & 18.50 $\pm$ 1.28  & 23.22 $\pm$ 0.29 \\
+ \model{}             &  \textbf{74.05 $\pm$ 3.04}  &   \textbf{75.84 $\pm$ 1.42}     &   \textbf{48.39  $\pm$  0.98}   &  \textbf{49.09  $\pm$  0.44}  & \textbf{31.69  $\pm$  3.50}  & \textbf{36.17  $\pm$ 0.72}  & \textbf{20.55  $\pm$  1.54} & \textbf{24.36  $\pm$  0.23} \\ \hline
Multi-Krum                   &  73.09 $\pm$ 2.41      &   75.03 $\pm$ 0.32   &  47.75 $\pm$ 0.56  & 47.83 $\pm$ 0.42  &  37.26 $\pm$ 0.43 &  38.54 $\pm$ 0.20 & 20.55 $\pm$ 3.25 & 23.30 $\pm$ 0.57       \\
+ \model{}                & \textbf{81.87 $\pm$ 1.48}  &  \textbf{82.77 $\pm$ 0.31}     & \textbf{53.15 $\pm$ 0.41}     &  \textbf{53.35 $\pm$ 0.21}  &    \textbf{38.98 $\pm$ 0.31}   & \textbf{39.48 $\pm$ 0.26} & \textbf{22.43 $\pm$ 1.95} & \textbf{24.36 $\pm$ 0.23}\\ \hline
ResidualBase               & 73.61 $\pm$ 3.40   & 75.10 $\pm$ 1.29      &  44.80 $\pm$ 0.47     & 45.13 $\pm$ 0.48  &   35.05 $\pm$ 1.59     &  38.60 $\pm$ 0.29  & 19.44 $\pm$ 2.60  & 23.86 $\pm$ 0.18 \\
+ \model{}             &  \textbf{79.28 $\pm$ 1.27} & \textbf{80.83 $\pm$  1.17}      &  \textbf{50.62 $\pm$ 0.37}    &  \textbf{50.98 $\pm$ 0.47}  &  \textbf{36.22 $\pm$  2.67}     &  \textbf{39.24 $\pm$  0.39} & \textbf{22.41 $\pm$  1.74} & \textbf{24.27 $\pm$  0.28}  \\ \bottomrule
\end{tabular}


}
\end{table*}

==> tables/attack_partial_info_std.tex <==
\begin{table*}[t!]
\caption{Performance results on classification accuracy with standard errors in Scenario-2 over four datasets. Our model brings non-trivial improvement for all server-side baseline algorithms for both last and best accuracy.}
\label{tab:main_result2_std}
\centering
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{LIE} & \multicolumn{2}{c|}{CIFAR-10} &  \multicolumn{2}{c|}{CIFAR-100} & \multicolumn{2}{c|}{TinyImageNet} & \multicolumn{2}{c}{FEMNIST} \\ 
                      & ~~ Last ~~  & ~~ Best ~~  &  ~~ Last ~~ & ~~ Best ~~  & ~~ Last ~~ & ~~ Best ~~ & ~~ Last ~~ & ~~ Best ~~  \\ \midrule
No Defense            &   73.40 $\pm$ 3.12    &  76.68 $\pm$ 1.05  &  48.99 $\pm$ 0.92 & 49.43 $\pm$ 0.59 & 35.07 $\pm$ 1.25 & 37.92 $\pm$ 0.17 & 20.07  $\pm$ 0.41 & 22.30  $\pm$ 0.94 \\
+ \model{}           & \textbf{79.69 $\pm$ 2.88} & \textbf{82.78 $\pm$ 0.47 } & \textbf{52.88  $\pm$ 0.93}  & \textbf{53.46 $\pm$  0.49} &  \textbf{37.61 $\pm$ 0.98}  &  \textbf{39.27 $\pm$  0.22}  & \textbf{21.87 $\pm$  1.69} & \textbf{24.03 $\pm$ 0.22} \\ \hline
Median               &	55.71 $\pm$ 6.73 & 64.80 $\pm$ 2.54 & 46.40 $\pm$ 0.96 & 47.12 $\pm$ 0.50 & 26.79 $\pm$ 3.14 & 36.67 $\pm$ 0.19 & 17.81 $\pm$ 3.23 & 23.15 $\pm$ 0.34\\
+ \model{}            	&  \textbf{60.58 $\pm$ 7.23} & \textbf{72.97 $\pm$ 1.65} &  \textbf{50.46  $\pm$ 1.58} & \textbf{52.25 $\pm$ 0.47}  & \textbf{33.42 $\pm$ 3.11} & \textbf{36.90 $\pm$ 3.23} & \textbf{20.58  $\pm$ 2.34}  & \textbf{23.39 $\pm$ 0.28}  \\ \hline
Trimmed Mean                &  39.19 $\pm$ 21.77     & 76.29 $\pm$ 0.59   &  47.45 $\pm$ 0.47 & 47.77  $\pm$ 0.14 &  33.15 $\pm$ 2.25 & 35.87 $\pm$ 0.42 & 19.01 $\pm$ 0.12 & 22.21 $\pm$ 0.69 \\
+ \model{}           	  &    \textbf{42.86 $\pm$ 25.25}    &   \textbf{79.37 $\pm$ 0.91}   &  \textbf{51.48 $\pm$ 0.94}  & \textbf{51.91 $\pm$ 0.65}  & \textbf{35.70 $\pm$ 1.49}  &   \textbf{37.28 $\pm$ 0.21} & \textbf{21.67 $\pm$ 2.39} & \textbf{23.73 $\pm$ 0.21}\\ \hline
Norm Bound          	  &  12.30 $\pm$ 2.98       &  27.90 $\pm$ 1.56     &  47.42 $\pm$ 0.70   & 47.77 $\pm$ 0.48   &  32.43 $\pm$ 1.72  & 35.45  $\pm$ 0.53 & 20.50  $\pm$ 1.98  & 22.70  $\pm$ 0.75 \\
+ \model{}             &  \textbf{14.00 $\pm$ 3.96}  &   \textbf{38.34 $\pm$ 3.40}     &   \textbf{52.15   $\pm$  0.61}   &  \textbf{52.76 $\pm$  0.40}  & \textbf{35.59  $\pm$  1.08}  & \textbf{37.42   $\pm$ 0.30}  & \textbf{21.64  $\pm$  2.41} & \textbf{23.79 $\pm$  0.52} \\ \hline
Multi-Krum                   &  41.46 $\pm$ 24.82      &   75.80 $\pm$ 1.01   &  48.23  $\pm$ 0.57  & 48.66 $\pm$ 0.48  &  33.38 $\pm$ 1.43 &  36.32 $\pm$ 0.17 & 20.25 $\pm$ 1.40 & 22.43 $\pm$ 0.71       \\
+ \model{}                & \textbf{46.30  $\pm$ 25.66}  &  \textbf{79.05 $\pm$ 0.79}     & \textbf{51.79 $\pm$ 1.08}     &  \textbf{52.57 $\pm$ 0.51}  &    \textbf{35.22 $\pm$ 1.26}   & \textbf{37.04 $\pm$ 0.09} & \textbf{21.93 $\pm$ 1.10} & \textbf{23.44 $\pm$ 0.15}\\ \hline
ResidualBase               & 74.53 $\pm$ 2.58   & 77.04 $\pm$ 0.64      &  48.68 $\pm$ 0.57     & 48.88 $\pm$ 0.47  &   33.61 $\pm$ 2.17     &  38.21 $\pm$ 0.19  & 20.21 $\pm$ 0.40  & 22.92 $\pm$ 1.00 \\
+ \model{}             &  \textbf{83.19 $\pm$ 1.09} & \textbf{83.65 $\pm$  0.40}      &  \textbf{53.11 $\pm$ 1.03}    &  \textbf{53.55 $\pm$ 0.65}  &  \textbf{36.73 $\pm$  1.24}     &  \textbf{38.73 $\pm$  0.40} & \textbf{22.66 $\pm$  1.63} & \textbf{24.01 $\pm$  0.27}  \\ \bottomrule
\end{tabular}

\vspace{0.5cm}

\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{STAT-OPT} & \multicolumn{2}{c|}{CIFAR-10} &  \multicolumn{2}{c|}{CIFAR-100} & \multicolumn{2}{c|}{TinyImageNet} & \multicolumn{2}{c}{FEMNIST} \\ 
                      & ~~ Last ~~  & ~~ Best ~~  &  ~~ Last ~~ & ~~ Best ~~  & ~~ Last ~~ & ~~ Best ~~ & ~~ Last ~~ & ~~ Best ~~  \\ \midrule
No Defense            &   73.74 $\pm$ 1.56    &  73.99 $\pm$ 1.23  &  23.40  $\pm$ 0.37 & 24.16 $\pm$ 0.36  & 26.82 $\pm$ 0.35 & 26.82 $\pm$ 0.35 & 19.67 $\pm$ 1.02 & 22.43   $\pm$ 0.70 \\
+ \model{}           & \textbf{79.77 $\pm$ 2.04} & \textbf{80.46 $\pm$ 0.91 } & \textbf{29.49 $\pm$ 0.26}  & \textbf{29.49 $\pm$  0.26} &  \textbf{29.62 $\pm$ 0.54}  &  \textbf{29.62 $\pm$  0.54}  & \textbf{21.68 $\pm$  1.38} & \textbf{24.13  $\pm$ 0.23} \\ \hline
Median               &	53.37 $\pm$ 5.93 & 58.17 $\pm$ 2.13 & 16.95 $\pm$ 0.45 & 17.02 $\pm$ 0.33 & 18.27 $\pm$ 0.75 & 18.39 $\pm$ 0.59 & 10.56 $\pm$ 0.50 & 14.60 $\pm$ 1.10 \\
+ \model{}            	&  \textbf{60.88 $\pm$ 4.53} & \textbf{66.01 $\pm$ 0.83} &  \textbf{23.21 $\pm$ 0.75} & \textbf{23.62 $\pm$ 0.42}  & \textbf{21.68 $\pm$ 0.91} & \textbf{23.63 $\pm$ 0.63} & \textbf{15.02  $\pm$ 2.54}  & \textbf{19.16 $\pm$ 0.10}  \\ \hline
Trimmed Mean                &  64.46 $\pm$ 3.87     & 68.34 $\pm$ 1.54   &  25.24 $\pm$ 0.28 & 25.27 $\pm$ 0.25 &  26.52 $\pm$ 0.58 & 26.54 $\pm$ 0.56 & 19.48 $\pm$ 0.76 & 22.83 $\pm$ 0.68 \\
+ \model{}           	  &    \textbf{82.53 $\pm$ 1.08}    &   \textbf{83.05 $\pm$ 0.33}   &  \textbf{29.80 $\pm$ 0.39}  & \textbf{29.89 $\pm$ 0.33}  & \textbf{27.26 $\pm$ 0.61}  &   \textbf{27.29 $\pm$ 0.56} & \textbf{21.99 $\pm$ 1.49} & \textbf{24.24 $\pm$ 0.25}\\ \hline
Norm Bound          	  &  64.15 $\pm$ 2.32       &  64.70 $\pm$ 1.71     &  23.61 $\pm$ 0.50   & 23.66 $\pm$ 0.44   &  23.61 $\pm$ 0.55  & 23.70 $\pm$ 0.43 & 19.14 $\pm$ 1.22  & 21.97 $\pm$ 0.36 \\
+ \model{}             &  \textbf{82.45 $\pm$ 0.85}  &   \textbf{82.85 $\pm$ 0.34}     &   \textbf{30.45 $\pm$  0.32}   &  \textbf{30.60 $\pm$  0.06}  & \textbf{26.66  $\pm$  0.63}  & \textbf{26.66 $\pm$ 0.63}  & \textbf{21.59  $\pm$  0.58} & \textbf{24.15 $\pm$  0.25} \\ \hline
Multi-Krum                   &  75.56 $\pm$ 1.64      &   76.10 $\pm$ 1.23   &  25.34 $\pm$ 0.29  & 25.62 $\pm$ 0.16  &  26.39 $\pm$ 0.66 &  26.40 $\pm$ 0.64 & 19.88 $\pm$ 1.25 & 23.16 $\pm$ 0.32       \\
+ \model{}                & \textbf{82.33 $\pm$ 1.05}  &  \textbf{82.80 $\pm$ 0.46}     & \textbf{31.42 $\pm$ 0.54}     &  \textbf{31.52 $\pm$ 0.44}  &    \textbf{27.83 $\pm$ 0.38}   & \textbf{27.95 $\pm$ 0.22} & \textbf{22.06 $\pm$ 1.17} & \textbf{24.16 $\pm$ 0.11}\\ \hline
ResidualBase               & 70.24 $\pm$ 1.72   & 70.39 $\pm$ 1.58      &  26.46 $\pm$ 0.34     & 26.57 $\pm$ 0.21  &   28.10 $\pm$ 0.56     &  28.10 $\pm$ 0.56  & 19.07 $\pm$ 1.35  & 21.53 $\pm$ 0.42 \\
+ \model{}             &  \textbf{77.81 $\pm$ 2.26} & \textbf{78.73 $\pm$  0.74}      &  \textbf{31.41 $\pm$ 0.34}    &  \textbf{31.41 $\pm$ 0.34}  &  \textbf{28.49 $\pm$  0.35}     &  \textbf{28.51 $\pm$  0.36} & \textbf{22.01 $\pm$  1.61} & \textbf{23.97 $\pm$  0.39}  \\ \bottomrule
\end{tabular}

\vspace{0.5cm}

\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{DYN-OPT} & \multicolumn{2}{c|}{CIFAR-10} &  \multicolumn{2}{c|}{CIFAR-100} & \multicolumn{2}{c|}{TinyImageNet} & \multicolumn{2}{c}{FEMNIST} \\ 
                      & ~~ Last ~~  & ~~ Best ~~  &  ~~ Last ~~ & ~~ Best ~~  & ~~ Last ~~ & ~~ Best ~~ & ~~ Last ~~ & ~~ Best ~~  \\ \midrule
No Defense            &   62.37 $\pm$ 1.76    &  63.13 $\pm$ 0.74  &  49.33 $\pm$ 0.66 & 49.70 $\pm$ 0.27  & 30.66 $\pm$ 0.33 & 30.66 $\pm$ 0.33 & 19.41 $\pm$ 0.35 & 22.63  $\pm$ 0.82 \\
+ \model{}           & \textbf{68.78 $\pm$ 1.68} & \textbf{69.53 $\pm$ 0.83 } & \textbf{53.86 $\pm$ 0.43}  & \textbf{54.21 $\pm$  0.21} &  \textbf{32.50 $\pm$ 0.48}  &  \textbf{32.52 $\pm$  0.44}  & \textbf{21.42 $\pm$  1.58} & \textbf{24.29 $\pm$ 0.23} \\ \hline
Median               &	74.71 $\pm$ 2.07 & 76.65 $\pm$ 0.36 & 46.81 $\pm$	0.53 & 46.91 $\pm$ 0.39 & 20.12 $\pm$ 0.95 & 20.33 $\pm$ 0.73 & 19.14 $\pm$ 0.94 & 22.52 $\pm$ 0.89\\
+ \model{}            	&  \textbf{81.86 $\pm$ 1.59} & \textbf{83.07 $\pm$ 0.55} &  \textbf{51.11 $\pm$ 0.72} & \textbf{51.49 $\pm$ 0.30}  & \textbf{23.65 $\pm$ 0.62} & \textbf{23.89 $\pm$ 0.68} & \textbf{21.01 $\pm$ 1.92}  & \textbf{24.16 $\pm$ 0.15}  \\ \hline
Trimmed Mean                &  72.80 $\pm$ 2.78     & 75.18 $\pm$ 0.88   &  47.80 $\pm$ 0.47 & 47.87 $\pm$ 0.40 &  26.40 $\pm$ 0.53 & 26.47 $\pm$ 0.45 & 18.19 $\pm$ 0.79 & 21.71 $\pm$ 0.31 \\
+ \model{}           	  &    \textbf{81.29 $\pm$ 1.69}    &   \textbf{82.18 $\pm$ 0.58}   &  \textbf{52.64 $\pm$ 0.60}  & \textbf{52.86 $\pm$ 0.37}  & \textbf{31.42 $\pm$ 0.34}  &   \textbf{31.48 $\pm$ 0.29} & \textbf{20.70 $\pm$ 1.83} & \textbf{23.77 $\pm$ 0.29}\\ \hline
Norm Bound          	  &  72.54 $\pm$ 3.14       &  75.09 $\pm$ 1.50     &  47.83 $\pm$ 0.46   & 48.01 $\pm$ 0.35   &  27.17 $\pm$ 0.41  & 27.19 $\pm$ 0.38 & 19.55 $\pm$ 1.30  & 22.25 $\pm$ 0.41 \\
+ \model{}             &  \textbf{81.47 $\pm$ 1.64}  &   \textbf{82.42 $\pm$ 0.32}     &   \textbf{53.09  $\pm$  0.42}   &  \textbf{53.19  $\pm$  0.32}  & \textbf{31.45  $\pm$  0.46}  & \textbf{31.49  $\pm$ 0.38}  & \textbf{20.89  $\pm$  1.82} & \textbf{23.88  $\pm$  0.39} \\ \hline
Multi-Krum                   &  71.49 $\pm$ 3.20      &   75.25 $\pm$ 0.59   &  48.23 $\pm$ 0.37  & 48.41 $\pm$ 0.30  &  26.31 $\pm$ 0.40 &  26.31 $\pm$ 0.40 & 19.56 $\pm$ 1.51 & 22.82 $\pm$ 0.58       \\
+ \model{}                & \textbf{80.94 $\pm$ 2.22}  &  \textbf{82.43 $\pm$ 0.14}     & \textbf{52.96 $\pm$ 0.43}     &  \textbf{53.23 $\pm$ 0.27}  &    \textbf{31.34 $\pm$ 0.38}   & \textbf{31.44 $\pm$ 0.22} & \textbf{20.96 $\pm$ 1.28} & \textbf{23.87 $\pm$ 0.19}\\ \hline
ResidualBase               & 74.40 $\pm$ 2.39   & 76.93 $\pm$ 0.80      &  48.96 $\pm$ 0.25     & 49.03 $\pm$ 0.21  &   27.93 $\pm$ 0.43     &  27.96 $\pm$ 0.43  & 19.28 $\pm$ 0.45  & 23.08 $\pm$ 0.94 \\
+ \model{}             &  \textbf{83.48 $\pm$ 0.88} & \textbf{83.90 $\pm$  0.32}      &  \textbf{54.39 $\pm$ 0.41}    &  \textbf{54.70 $\pm$ 0.33}  &  \textbf{31.85 $\pm$  0.46}     &  \textbf{31.88 $\pm$  0.40} & \textbf{21.49 $\pm$  1.57} & \textbf{24.15 $\pm$  0.15}  \\ \bottomrule
\end{tabular}



\end{table*}

